Synthesizing Invariants for Polynomial Programs by Semidefinite Programming

Constraint-solving-based program invariant synthesis takes a parametric invariant template and encodes the (inductive) invariant conditions into constraints. The problem of characterizing the set of all valid parameter assignments is referred to as the strong invariant synthesis problem, while the problem of finding a concrete valid parameter assignment is called the weak invariant synthesis problem. For both problems, the challenge lies in solving or reducing the encoded constraints, which are generally non-convex and lack efficient solvers. Consequently, existing works either rely on heuristic optimization techniques (such as bilinear matrix inequalities) or resort to general-purpose solvers (such as quantifier elimination), leading to a trade-off between completeness and efficiency. In this paper, we propose two novel algorithms for synthesizing invariants of polynomial programs using semidefinite programming (SDP): (1) The Cluster algorithm targets the strong invariant synthesis problem for polynomial invariant templates. Leveraging robust optimization techniques, it solves a series of SDP relaxations and yields a sequence of increasingly precise under-approximations of the set of valid parameter assignments. We prove the algorithm's soundness, convergence, and weak completeness under a specific robustness assumption on templates. Moreover, the outputs can simplify the weak invariant synthesis problem. (2) The Mask algorithm addresses the weak invariant synthesis problem in scenarios where the aforementioned robustness assumption does not hold, rendering the Cluster algorithm ineffective. It identifies a specific subclass of invariant templates, termed masked templates, involving parameterized polynomial equalities and known inequalities. By applying variable substitution, the algorithm transforms constraints into an equivalent form amenable to SDP relaxations.

==> response/response.tex <==
the responses can be found via 

https://www.overleaf.com/7718777419rnwyqcwmtyys#d74fb6


% \documentclass{article}

% % Language setting
% % Replace `english' with e.g. `spanish' to change the document language
% \usepackage[english]{babel}

% % Set page size and margins
% % Replace `letterpaper' with`a4paper' for UK/EU standard size
% \usepackage[letterpaper,top=2cm,bottom=2cm,left=3cm,right=3cm,marginparwidth=1.75cm]{geometry}

% % Useful packages
% \usepackage[colorlinks=true, allcolors=blue]{hyperref}


% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{graphicx}
% \usepackage{amsfonts}
% \usepackage{verbatim}
% \usepackage{times}
% \usepackage{multirow}
% \usepackage{bbm}
% \usepackage{amsthm}
% \usepackage{stmaryrd}
% \usepackage{algorithm}
% \usepackage[algo2e,norelsize,  ruled, lined, boxed, commentsnumbered]{algorithm2e}


% \title{
% Response to Reviewers\\
% }

% \author{Hao Wu \and 
% Qiuye Wang \and
% Bai Xue \and
% Naijun Zhan \and
% Lihong Zhi \and
% Zhihong Yang
% }


% \begin{document}
% \maketitle

% \noindent Dear editor and reviewers,

% % thank you for your diligent review of our previous version entitled with  ``Synthesizing Invariant Clusters for Polynomial Programs by Semidefinite Programming'', which was submitted to TOPLAS last year.
% % Your insightful comments have been invaluable in improving the quality and contribution of our work. 
% % We are sincerely grateful for your time and effort invested in this review process.

% % We would like to inform of you that the current version made a substantial revision and expansion of our previous work.
% % Based on your review reports, we conducted a comprehensive revision, involving the following major changes:

% \begin{enumerate}
%     \item \textbf{Problem Formulation} In Section~2 and Section~3, we have added a lot of technical details for better clarity and readability. 
    
%     \item \textbf{Technical Details} In Section~2 and Section~3, we have added a lot of technical details for better clarity and readability. 
%     \item \textbf{Presentation} In Section~4, In Section~5 explanation.
%     \item \textbf{A new completeness result for masked templates}
%     \item \textbf{Experiments}
% \end{enumerate}


% \section{Responses}
% \input{response/review1}
% \input{response/review2}
% \input{response/review3}



% \end{document}

==> response/review1.tex <==
%!TEX root = response/response.tex
\subsection{Responses to Reviewer 1}
\begin{itemize}

\item \textbf{Comment R1.1} 
\textit{
It is worth noting that the authors’ hyper-rectangles are bounded. If I am correct, compactness is fundamental to Putinar’s Positivstellensatz (with its requirements for convergence results in measurable spaces).
}

In fact, the boundedness constraint is not essential in applying Putinar's Positivstellensatz. Some recent works in polynomial optimization have removed this restriction, by using polynomial homogenization [34] or Putinar-Vasilescu's Positivstellensatz [51]. In fact, we have another paper on how to apply homogenization in the context of invariant synthesis [78]. However, a deeper explanation on this topic needs many other notions that are not related to our invariant synthesis problem. We discuss this and give references in Remark 1.
See Page 6, line 266-273.

\item \textbf{Comment R1.2} 
\textit{
On the one hand, the authors have omitted the proofs of several results. On the other hand, they provide references to the literature. The choice likely benefits the readability, but hinders a dedicated reader.
}

We have reformulated the presentation in our technical part and supplied many details. Now we only omit the proof of convergence (Thm.5 in section 3). This is because the proof is based on measure theory and is essentially the same as in the cited paper.   
 
\item \textbf{Comment R1.3} 
\textit{
The authors use boldface fonts to indicate vector-valued polynomials and vectors (Preliminaries 2), but do not use boldface to indicate, say, the vector of zeros. (See, for instance, the many component-wise polynomial inequalities in Code 1 on page 4.)
}

Thank you for your suggestions. We change constant vectors to bold symbols in our formulas. We also modify some other notations for better clarity.

\item \textbf{Comment R1.4} 
\textit{
On page 22, the authors make a comparison between recurrence-based approaches to invariant synthesis and the Skolem Problem (with a citation to [47]). I find the claim that the two problems are closely related to be spurious at best and disingenuous at worst. [47] is groundbreaking work on the Skolem Problem, but makes no mention of invariant synthesis. I note that works in the literature that consider recurrence analysis as an approach to computing algebraic invariants, such as [https://arxiv.org/abs/2307.10902], do exist.  
}

Response: Many thanks! Apparently, this is a more appropriate reference for our claim. We have amended this mistake.
See Page 28, Line 1349-1351.

\end{itemize}

==> response/review2.tex <==
\subsection{Responses to Reviewer 2}
\begin{itemize}

\item \textbf{Comment R2.1} 
\textit{
My main concern is how the novelty of this submission compares with the prior work that is reference [13] in the submission and its extension [29]? My understanding is that the submission and [13, 29] give similar contributions in that both techniques synthesize polynomial inequality invariants, using a sum-of-squares relaxation via Putinar’s Positivstellensatz, to achieve a degree-bounded completeness result. Both techniques reduce the invariant synthesis problem to SDP ([13, 29] uses quadratic programming more specifically). [13->14, 29->28]
}

Response: Putinar's Positivstellensatz is a standard technique in reasoning about nonlinear real arithmetic. Both this work and [14, 28] utilize this theorem to transform the original invariant conditions into constraints involving SOS polynomials. 

The main issue here is that the transformed constraints can not be directly solved as SDPs.  To be exact, the resulting constraints are bilinear matrix inequalities, or equivalently, (nonconvex) quadratic programming. Solving such constraints is NP-hard in general, while SDP can be solved in polynomial time. See Remark 2 for a detailed explanation. Page 8, line 380.

The main contribution of [14, 28] is a systematic procedure to encode the invariant synthesis problem (and also program synthesis problem [28]) of a program into quadratic programming. After that, they rely on tools like Z3 to solve the constraints. In contrast, our main contribution is the new SDP-based algorithms for solving the constraints.


\item \textbf{Comment R2.2} 
\textit{
The submission takes a roundabout path to generate an invariant compared with [13, 29], by generating an invariant cluster and then an invariant from the cluster. This alternative path may be advantageous in that it ultimately results in an easier query for a solver to handle. If this is the motivation for the submission it needs to be discussed in the introduction or the main body of the paper, rather than in the related work. 
}

Thanks for your comment. Now we have reclarified our contributions in a different way. The Cluster algorithm provides under-approximations to the strong invariant synthesis problem. As a byproduct, its solution can be directly used to simplify the weak invariant synthesis problem. 

 
\item \textbf{Comment R2.3} 
\textit{
Comment 2.3: I would like an explanation or some intuition on why your method is so much more performant, when to my eye the submission and [13,29] seem so similar. This explanation might be quite simple, but I find it’s lacking in the current draft.  
}

The reason is that solving convex optimization problems (such as SDP) is much easier than solving non-convex optimization problems (such as quadratic programming or bilinear matrix inequalities). Although there exists many optimizers/solvers for non-convex problems, their capacity is rather limited.
Generally speaking, the invariant synthesis problem is hard because it is essentially non-convex (due to the inductiveness condition). And our work is dedicated to ``convexify'' the constraints.

\item \textbf{Comment R2.4} 
\textit{
I think it would be helpful to be more explicit with the algorithms, especially in the experiments section. You refer to two algorithms in the experiments section. I’m assuming this is the base algorithm and the masked templates algorithm. Do you use the binary search algorithm (Algorithm 1) in the experimental evaluation? 
}

Thanks for your suggestion. Now we call the algorithm in Section 3 and Section 4 the Cluster algorithm, and the algorithm in Section 5 the Mask algorithm.
The binary search strategy is not used in our experiments because it can fail due to numerical errors. 
To avoid such confusion, we replace it by a concrete example in Section 4.1 and left the strategy in appendix.

\item \textbf{Comment R2.5} 
\textit{
I was confused in the experiments section when you said nested loops are not supported. However, the extension in section 4 is exactly for this case. If this is presented as a contribution, I think it needs to be experimentally evaluated.
}

Our Cluster algorithm supports nested loops, while the Mask algorithm do not. So we exclude those benchmarks containing nested loops in Mask benchmarks.


\item \textbf{Comment R2.6} 
\textit{
How is the time calculated in the experiments?  Does the time for your method include the Posterior Verification time described on line 962? 
}

For all benchmarks, the verification (whether an invariant is valid) can be done within 0.1 seconds using Z3, which is dominated by the time needed to solve the constraints.
Page 27, line 1282.

\item \textbf{Comment R2.7} 
\textit{
My understanding is that QP and Z3 are exact and thus the invariant they produce is an invariant, but yours may not be due to numerical errors. I think a more fair comparison would be to include the posterior verification if that time is not already included. 
}


\item \textbf{Comment R2.8} 
\textit{
In relation to the previous question, does the calculation of time explain why the times you report for QP differ so significantly from what they present in their paper? For example, you report QP timing out on the mannadiv example, but they report their technique took 5.25 seconds.
}

Different task, different template
See Remark 4 on Page 24, line 1158.



\end{itemize}

==> response/review3.tex <==
\subsection{Responses to Reviewer 3}

\begin{itemize}

\item \textbf{Comment R3.1} 
\textit{
In some places, the paper mentions that existing techniques face a trade-off and rely on general-purpose solvers, alluding that this would be a disadvantage. However, the presented approach also relies on out-of-the-box (SDP/numerical) solvers. It also uses Z3 in an example. Why is the author’s approach not subject to the same trade-offs? Isn’t the presented approach also based on templates and approximations that require some trade-offs?
}

Response: 
Of course, our algorithm (and any algorithm in any field) subjects to the trade-off between expressiveness and  efficiency. Our intention here is to say that our method does not suffer from this tradeoff as severe as existing methods, since each constrain we solve is an SDP. To hightlight this point, we add the word "severe" is this sentence, see Page 1, line 16.


\item \textbf{Comment R3.2} 
\textit{
Line 53. The informal description of inductive invariants does not adequately highlight inductivity. A non-inductive invariant also continues to hold (since it’s invariant).
}

Response: Thanks, we rephrase our statement as follows: An inductive invariant is a specific type of invariants that satisfies the inductive property: if the assertion holds at a program location, then it is preserved during subsequent visits to that location, see Page 2, line 51.


\item \textbf{Comment R3.3} 
\textit{
L74. Why "quantified" (and not just FOL formula)? Do you mean "with quantifiers"?
}

Response: Yes, we want to highlight that the constraints have alternative quantifiers (there exists parameters such that for all program variables). We have rephrased this sentence to avoid confusion. See Page 2, line 73-84.

\item \textbf{Comment R3.4} 
\textit{
Line 75, The statement about decidability is quite misleading. Up to this point, the paper never states that variables are real-valued. If they would be integer-valued, the problem would be undecidable. If the ongoing assumption is that all variables are real-valued, this should be made clear early on, e.g., in line 70, by stating that the paper considers polynomial programs over real-valued variables. Related to that, it should also be clarified that whenever the authors refer to SMT, they mean reasoning about non-linear real arithmetic. This is never explicitly mentioned.
}

Response: Yes, we totally agree with you. We did forget to state that program variables are real-valued at this point. Now we add this requirement at the beginning of this paragraph, see Line 69. We also clarify on general-purpose solvers later in this paragraph, following your suggestions. See Page 2, line 73-84.

\item \textbf{Comment R3.5} 
\textit{
Line 81, The paper should properly introduce SDP, which has only been mentioned in the abstract.
}

Response: Thanks for your suggestion. Now we introduce SDP in the preliminaries (Sec 2.1) and explain how to translate a SOS program into an SDP. See Page 5, line 230.

\item \textbf{Comment R3.6} 
\textit{
More general than what? This characterization sounds like many constrained based approaches. How is the characterization of all solutions leveraged? After further reading, the approach requires a set of solutions because the completeness theorem relies not only on the existence of one invariant in the search space given by the template but a set of solutions (i.e., an interior point).
}




\item \textbf{Comment R3.7} 
\textit{
Comment 3.7: l. 85: Does the constraint have to hold for some or all d? The text later suggests some (sufficiently large)?
}

For each $d$, the polynomial $h_d(\bm{a})$ is an under-approximation of the valid set. 
However, it could be the case that $h_d(\bm{a})\le 0$ has no solution.
semi-completeness reuslt

\item \textbf{Comment R3.8} 
\textit{
l. 86, first contribution para: I fear this makes the paper hard to many TOPLAS readers. Could you better explain what having an interior point means in this setting and the consequences? At first glance, it seems to go beyond having an actual loop invariant among the template instances. after reading section 5, I have also become quite critical because the requirement seems to rule out the presence of logical variables unless one introduces masked templates.
}

Section 5.1

\item \textbf{Comment R3.9} 
\textit{
l. 91, Why are equalities not supported by the first approach? This was a bit surprising and is another point why the results need to be phrased in a way that is more accessible to the community
}

Section 5.1

\item \textbf{Comment R3.10} 
\textit{
I guess g(x), c(x), and f(x) must be polynomials or ions? It would be good to state this explicitly.
}

Page 7, line 295.

\item \textbf{Comment R3.11} 
\textit{
Assumption 1: Just for clarification: This assumption is only needed for the weak completeness result? 
Could one incorporate it into the invariants rather than assuming it? 
Would the approach remain sound without the assumption?
}

Response: Yes, the assumption is just needed for completeness and both our approaches remain sound without it. This is also the case for [] and []. In fact, this assumption is not essential both in theory and in practice. As discussed in Remark?, we can remove this assumption by using extensions of Putinar's Positivstellenstaz. In experiments, the boundness restriction also has very little impact on results.

\item \textbf{Comment R3.12} 
\textit{
Assumption 2: The part about numerical solvers raises the question of what kind of soundness guarantee one actually obtains from this approach. Would this assumption be necessary if we had an exact solver over reals (not floats)? (I understand that this is a somewhat common assumption nonetheless.)
}

Response: The answer is yes, because we only use this assumption to strengthen the invariant conditions. Namely, in Eq.(8), we change $g>0$ (written as $\neg g<=0$)to $g>=0$. We now emphasis that both the assumptions are made for completeness.

See Page 7, line 323.

\item \textbf{Comment R3.13} 
\textit{
The problem formulation in 2.2 is quite clear but the development in 2.3 seems unconnected on a first read. It would be nice to have a clearer outline of the overall approach.
}

Response: We now change the order of subsections in preliminaries. We first introduce SOS relaxation technique and use it to explain the challenge in invariant synthesis.
Section 2

\item \textbf{Comment R3.14} 
\textit{
l. 249 “defining polynomials” has not been explained/introduced; strictly speaking, even “strictly positive” is undefined 
}

Response: Thank you for pointing out. We have rephrased the paragraph (and some other sentences in the paper) to avoid undefind notions.

\item \textbf{Comment R3.15} 
\textit{
l. 253 inconsistent usage of semi-algebraic sets; according to sec. 2, it should be p_i(x) <= 0; I realize that this representation is standard for Putinar’s theorem. However, it also affects the examples, where (4) states p_i(x) <= 0.
}

Response: For simplicity, we just change the definition of basic semialgebraic sets to allow for >,>=,<=,<. It really depends on the context which notation is more convenient. See Page 3, line 139.

\item \textbf{Comment R3.16} 
\textit{
While I can follow the example on page 6, I believe its presentation needs to be improved to be comprehensible to a broader readership. In particular, the example does not really demonstrate how Putinar’s theorem is applied (or rather: it leaves significant intermediate steps to the reader). In particular, “transform into the program” is not clear. In what relation do these transformations stand? Are these approximations (as in the step from (5) to (6))? Are these equivalent? This whole page leaves too much to the reader for an initial example. It is also left to the reader to exploit linearity of l(a,x).
}

Response: We have supplied technical details on SOS relaxations. We believe that your questions can be answered by Section 2.1.

\item \textbf{Comment R3.17} 
\textit{
The paper does not explicitly state what a semindefinite programming problem is. There is certainly enough space in a Journal article to define one of the core techniques the paper relies upon. Instead, even the first simple example is somewhat opaque (e.g. “(6) can be transformed into an SDP […] using interior-point methods”). Again, I doubt this is accessible to the general TOPLAS readership who might be interested in those techniques.
}

Response: The same as the above response.

\item \textbf{Comment R3.18} 
\textit{
Comment 3.18: I can understand how we end up with (10) but the “distance” between those steps is generally too large. The paper jumps around between objectives, and there is little explanation of why and how, or even what is approximated/equivalent in what way to the previous problem. It’s hard to follow how we end up with the sum in (11). I understand it follows the idea of [43, Sec. 3.3], but this is barely accessible to a reader of this paper.
}

Response: Section 3.3.

\item \textbf{Comment R3.19} 
\textit{
Comment 3.19: l. 376: Why k+2 if there are k branches?
}

k branches, precondition and postcondition.

\item \textbf{Comment R3.20} 
\textit{
Comment 3.20: l. 381: the constant M seems arbitrary and magical. Please explain.
}

We now set $M=-1$. In theory, it can be any negative constant. 

\item \textbf{Comment R3.21} 
\textit{
Comment 3.21: p. 9, (14) - (19): While I can identify how the invariant conditions are mapped to an SDP here, the paper could do a better job of guiding a reader and explaining the structure of the constructed SDP. Right now, a reader must reconstruct (14) - (16) and what this states about the original invariant conditions.
}



\item \textbf{Comment R3.22} 
\textit{
Comment 3.22: I do not understand remark 4. In what sense does the described technique yield a cluster of invariants instead of one invariant? Because there is an interior point and we can those add small constants and still obtain an invariant? Is the solution a to h^(d)(a) <= 0 symbolic? Or does this refer to the fact that we could search for multiple solutions to the constraint? 
}


\item \textbf{Comment R3.23} 
\textit{
Comment 3.23: I understand that Theorem 4 is an instance [43, Theorem 3]. However, the conditions are meaningless for readers familiar with invariant synthesis but not SDP. I appreciate the discussion following Theorems 4 and 5, but this does not give sufficient intuition. It just tries to assure readers that “these conditions are rarely violated” without much evidence. On this note, what does “relatively rare in theory” mean?
}

reformulate, explain using Assumption 2 and the finite convergence property of Putinar's theorem.
Page 13, 615-632.

\item \textbf{Comment R3.24} 
\textit{
Comment 3.24: l. 425: How can you back up claims like “In most cases, it can be efficiently solved by modern symbolic solvers”? 
The experiments do not even seem to use a symbolic solver with exact arithmetic!
}

\item \textbf{Comment R3.25} 
\textit{
Comment 3.25: l. 449: Interior points are not defined.
}

Page 3, line 139-140.


\item \textbf{Comment R3.26} 
\textit{
Comment 3.26: Why is Lemma 1 introduced at this point? It’s also misleading because J(a) has been overloaded in (12).
}


\item \textbf{Comment R3.27} 
\textit{
Comment 3.27: l. 467 onwards is very confusing. What is J(a) referring to? As defined in (9), as  indicated in Lemma 1, or as in (13), given the discussion of invariants. Lemma one also seems irrelevant for the discussion (if it is not, please make this explicit).
}

\item \textbf{Comment R3.28} 
\textit{
Comment 3.28: Example 1: Settong g(x) = 0 would mean the loop never terminates. Please change the example such that it matches Code 1. It is disturbing that the first concrete example deviates from the proposed form. The example misses the opportunity to clarify open questions about the sum of square relaxations. Why do you not provide the concrete constraints (meaning: instances of 14 - 17 each) for this concrete example? This would significantly help a reader, particularly those familiar with other synthesis techniques. In its current state, the example is not helpful to gain a better intuition on the provided approach. Without seeing the detailed constraints that are solved here, it is hard to judge why the formulation of synthesis proposed by this paper is indeed simpler, as claimed.
}

Page 14, line 647-657.

\item \textbf{Comment R3.29} 
\textit{
Comment 3.29: Is the part about nested loops a special case of supporting semi-algebraic templates for a slightly more complex loop?
}

Response: Not really, the constraints are of different shapes. 

\item \textbf{Comment R3.30} 
\textit{
Comment 3.30: this also does not directly match Code 1 (although the transformation is trivial)
}

Page 27, line 997-1007.

\item \textbf{Comment R3.31} 
\textit{
Comment 3.31: I’m not sure I can follow the observation here. What does it mean for an “algorithmic program” to represent “strict symbolic relations”, also in the presence of Assumption 2?
}

Section 5.1

\item \textbf{Comment R3.32} 
\textit{
Comment 3.32: Is it correct to think of non-core variables as those that are never touched by a program (e.g. logical variables)? Is it important that those variables are also never read?
}

Definition 11, Page 20, line 970.

\item \textbf{Comment R3.33} 
\textit{
Comment 3.33: The last sentence in 769 is very important to my understanding. I was quite confused first in Def. 7 why R refers to all indices of non-core variables.
}

\item \textbf{Comment R3.34} 
\textit{
Why is “rounding off” sound?
}


\item \textbf{Comment R3.35} 
\textit{
Discussing these kinds of properties to gain an intuition would have been very valuable in the main part of the paper!
}

Section 5.1

\item \textbf{Comment R3.36} 
\textit{
L 871. This could be more explicit. The apparently good benchmarks are on a subset of the referenced collection.
}



\item \textbf{Comment R3.37} 
\textit{
Comment 3.37: The benchmarks taken from [58] considered by this paper seem to differ from those considered in [13]. Table 2 includes some additional ones but also omitted others (e.g. euclidex3). Why?
}

Response: The code of [13] is not publicly available, so do we do not know the details of their experiments.  
euclidex3 reasons about gcd(x,y)


\item \textbf{Comment R3.38} 
\textit{
Comment 3.38: Can you give any intuition on why perhaps Z3 tends to be better on some of the examples in Table 1?
}

Response: we guess that Z3 has some search strategies

\item \textbf{Comment R3.39} 
\textit{
The fact that the algorithms are numerical should be highlighted more. Initial examples are solved with Z3 and it is somewhat hidden (although dicussed in l. 927).
}

\item \textbf{Comment R3.40} 
\textit{
The soundness of [13] does not depend on boundedness. Is this also the case for your approach? Do you supply the boundedness also to QP? Could the performance be explained because boundedness is not assumed (or even heavily exploited as in the binary search)?
}

\item \textbf{Comment R3.41} 
\textit{
How comparable are the approaches, if QP, Z3, etc. are exact whereas your implementation is not? Could you also report numbers for a sound approach, as outlined on p. 20?
}

\item \textbf{Comment R3.42} 
\textit{
The comparison to [13,29] is not convincing unless the questions about experiments can be clarified. The main difference is the transfer of results from [43] to invariant synthesis. The experiments are then incomparable due to numerics. The validation step mentioned before is not discussed in the paper (or at least I did not spot it).
}

\item \textbf{Comment R3.43} 
\textit{
How do we know that the polynomial benchmark examples have interior points?
}

Response: This is a good question, and is very important for our completeness result. However, right now we do not have an efficient algorithm for deciding it. But the problem is decidable because it can be formulated as a FOL sentence in reals.

Section 5.1

\item \textbf{Comment R3.44} 
\textit{
I found the description of the implementation insufficient. Various aspects were unclear, e.g. the reliance on numerical solvers, whether the results sound, whether the results are validated with an exact solver, what the precision is (it seems to be 10^-5 but this is never mentioned).
}

\item \textbf{Comment R3.45} 
\textit{
Are some of the benchmarks parameterized? It would be interesting to see how large instances can be until one encounters a timeout.
}

Response: We add a parameterized example ...

\end{itemize}
